Origin of the Galactic Diffuse X-ray Emission: Iron K-shell Line Diagnostics

This paper reports detailed K-shell line profiles of iron (Fe) and nickel (Ni) of the Galactic Center X-ray Emission (GCXE), Galactic Bulge X-ray Emission (GBXE), Galactic Ridge X-ray Emission (GRXE), magnetic Cataclysmic Variables (mCVs), non-magnetic Cataclysmic Variables (non-mCVs), and coronally Active Binaries (ABs). For the study of the origin of the GCXE, GBXE, and GRXE, the spectral analysis is focused on equivalent widths of the Fe K$\alpha$, Fe He$\alpha$, and Fe Ly$\alpha$ lines. The global spectrum of the GBXE is reproduced by a combination of the mCVs, non-mCVs, and ABs spectra. On the other hand, the GRXE spectrum shows significant data excesses at the Fe K$\alpha$ and Fe He$\alpha$ line energies. This means that additional components other than mCVs, non-mCVs, and ABs are required, which have symbiotic phenomena of cold gas and very high-temperature plasma. The GCXE spectrum shows larger excesses than those found in the GRXE spectrum at all the K-shell lines of iron and nickel. Among them the largest ones are the Fe K$\alpha$, Fe He$\alpha$, Fe Ly$\alpha$, and Fe Ly$\beta$ lines. Together with the fact that the scale heights of the Fe K$\alpha$, Fe He$\alpha$, and Fe Ly$\alpha$ lines are similar to that of the central molecular zone (CMZ), the excess components would be related to high-energy activity in the extreme envelopment of the CMZ.

==> table-AS.tex <==
\begin{table*} % The best-fit lines from Active Stars
\caption{The best-fit parameters of mCVs, non-mCVs and ABs for model A.}
\label{tab:AS}
\smallskip
\footnotesize
\begin{center}	
 \begin{tabular}{lccccccc}
   \hline
 \hline   
&&\multicolumn{2}{c}{mCV} &\multicolumn{2}{c}{non-mCV}&\multicolumn{2}{c}{AB}\\
\hline
\multicolumn{8}{c}{Continuum}\\
\multicolumn{2}{l}{\NH~($10^{22}$~cm$^{-2}$)}&\multicolumn{2}{c}{14.7$\pm{1.5}$}&\multicolumn{2}{c}{0 (fix)}&\multicolumn{2}{c}{0 (fix)}\\
\multicolumn{2}{l}{Fe K edge$^{a}$} &\multicolumn{2}{c}{$0.05\pm0.01$} &\multicolumn{2}{c}{$0.08\pm0.04$} &\multicolumn{2}{c}{$0.02(<0.05)$}\\
\multicolumn{2}{l}{$kT_{\rm e}$ (keV)}&\multicolumn{2}{c}{$23.3^{+5.1}_{-3.7}$}&\multicolumn{2}{c}{10.7$\pm{1.7}$}&\multicolumn{2}{c}{$4.25\pm{0.18}$}\\
	\hline
			\multicolumn{8}{c}{Emission lines}\\
Line$^b$	&CE$^b$  & Flux$^c$ & EW$^f$ & Flux$^d$ & EW$^f$ & Flux$^e$ & EW$^f$\\
  	\hline
\KaTab		&6400  	&4.88$\pm{0.13}$&169$\pm5$ 	&0.26$\pm{0.02}$ &82$\pm7$		&0.49$\pm{0.09} $&28$\pm5$\\
\HeaTab	&6680	&3.19$\pm{0.12}$&118$\pm5$ 	&1.29$\pm{0.03}$ &451$\pm10$ 	&4.97$\pm{0.12}$&327$\pm8$ \\
\LyaTab    &6966	&1.52$\pm{0.11}$&60$\pm4$  	&0.44$\pm{0.02}$ &167$\pm9$ 	&0.60$\pm{0.09}$&45$\pm6$ \\
\KbTab		&7059   &0.61$^g$     	&25 					&0.07$^g$ &12 							&0.06$^g$  &5\\
\NiKaTab  &7490	&-&-&-&-	&-&-\\
\NiHeaTab &7771 	&0.48$\pm{0.17}$ &23$\pm8$ 	&0.12$\pm{0.03}$ &56$\pm14$	&0.53$\pm{0.13}$&55$\pm13$\\
\HebTab 	&7881 	&$<0.32$ &$<16$ 						&0.09$\pm{0.03}$ &43$\pm14$	&0.15$\pm{0.13}$ &17$\pm15$\\
\LybTab 	&8251 	&0.43$^{+0.13}_{-0.33}$ &22$^{+7}_{-17}$ 	& $<0.07$  & $<28$  					&0.16$\pm{0.10}$ &20$\pm14$\\
\HecTab	&8295 	& $<0.35$ & $<18$ 					&0.09$^{+0.03}_{-0.07}$& 50$^{+17}_{-39}$	&$<0.08$&$<13$\\
\LycTab 	&8700 	& $0.18\pm0.13$ & $10\pm7$ 	&0.06$\pm{0.03}$&34$\pm17$	&$<0.17$&$<24$\\
\hline
$\chi ^2$/d.o.f.  &   & \multicolumn{2}{c}{409/314}    & \multicolumn{2}{c}{297/274}     & \multicolumn{2}{c}{361/363} \\
\hline
\end{tabular}
\end{center}
\tablenotetext{}{Errors are one standard deviation (1 $\sigma$).}
\tablenotetext{a}{Absorption depth at 7.11 keV.}
\tablenotetext{b}{AtomDB 3.0.2 (http://www.atomdb.org/) and \cite{Wa05}. Unit is eV.}
\tablenotetext{c}{Unit is $10^{-7}$~photon~cm$^{-2}$~s$^{-1}$.}
\tablenotetext{d}{Unit is $10^{-8}$~photon~cm$^{-2}$~s$^{-1}$.}
\tablenotetext{e}{Unit is $10^{-9}$~photon~cm$^{-2}$~s$^{-1}$.}
\tablenotetext{f}{Unit is eV.}
\tablenotetext{g}{Fixed to 0.125$\times$\KaTab. }
\end{table*}


